Minimal covariance realization and system identification algorithm for a class of stochastic linear switched systems with i.i.d. switching

In this paper, we consider stochastic realization theory of Linear Switched Systems (LSS) with i.i.d. switching. We characterize minimality of stochastic LSSs and show existence and uniqueness (up to isomorphism) of minimal LSSs in innovation form. We present a realization algorithm to compute a minimal LSS in innovation form from output and input covariances. Finally, based on this realization algorithm, by replacing true covariances with empirical ones, we propose a statistically consistent system identification algorithm.

==> Deterministic_LPV-SSA_representation.tex <==
\subsection{Deterministic LPV-SSA representation}
\label{sect:real:red}
%In order to present the results of this paper, it is necessary to introduce the deterministic LPV-SSA.
%which will be used in the process of obtaining an asLPV-SSA representation in innovation form. 
%For this reason, we 
Recall from \cite{PetreczkyLPVSS,CoxLPVSS} that a deterministic LPV state-space representation with affine dependence (abbreviated as \emph{dLPV-SSA})
is a system of the form:
\begin{equation}
	\label{eqn:LPV_SSA:det} 
	\mathscr{S}\left\{\begin{aligned}
		&\mathrm{x}(t+1)=\sum_{i=1}^{\pdim} (\mathcal{A}_i\mathrm{x}(t)+\mathcal{B}_i\mathrm{u}(t))\mu_i(t), ~ \\
		&\mathrm{y}(t)=\mathcal{C}\mathrm{x}(t)+\mathcal{D}\mathrm{u}(t),
	\end{aligned}\right.
\end{equation}
where $\mathcal{A}_i, \mathcal{B}_i, \mathcal{C}, \mathcal{D}$ are matrices of suitable dimensions,  
$\mathrm{x}:\mathbb{Z} \rightarrow \mathbb{R}^{n_\mathrm{x}}$ is the state trajectory
$\mathrm{u}:\mathbb{Z} \rightarrow \mathbb{R}^{n_\mathrm{u}}$ is the input trajectory
$\mathrm{y}:\mathbb{Z} \rightarrow \mathbb{R}^{n_\mathrm{y}}$ is the output trajectory with finite support \footnote{a function $g:\mathbb{Z} \longrightarrow \mathbb{R}^p$ has a finite support, then it $\exists \; t_0 \in \mathbb{Z}$, such that $\forall \; t<t_0$, $g(t)=0$.}.
% In order to avoid technical problems, 
%we assume that $x,u,y$ all have finite support, i.e. there exist a $t_0 \in \mathbb{Z}$, such that
%x(s)=0,y(s)=0,u(s)=0$ for all $s < t_0$. 
We identify a dLPV-SSA of the form \eqref{eqn:LPV_SSA:det} with the tuple 
\begin{equation} 
\label{eqn:LPV_SSA:det_not} 
\mathscr{S}=(\{\mathcal{A}_{i},\mathcal{B}_{i}\}_{i=0}^{\pdim},\mathcal{C},\mathcal{D})
\end{equation}
%The number $\nx$ is called the dimension of $\mathscr{S}$. 

%\textcolor{red}{Manas: please make the notation consistent with tha of stochastic LPV-SSA, i.e. use $(\{A_{i},B_{i}\}_{i=0}^{\pdim},C,D)$ instead.} 
The \emph{sub-Markov function} of the dLPV-SSA  $\mathscr{S}$ 
is the function $M_{\mathscr{S}}:\Sigma^{*} \rightarrow \mathbb{R}^{n_\mathrm{y} \times n_\mathrm{u}}$, such
that for all $w \in \Sigma^{*}$, 
\begin{equation}\label{eqn:sub_markov}
	M_{\mathscr{S}}(w)=\left\{\begin{array}{ll}
		\mathcal{CA}_s\mathcal{B}_{\sigma}, \ \ & w=\sigma s, \, \sigma \in \Sigma, \, s \in \Sigma^{*} \\
		\mathcal{D}.           \ \  & w=\epsilon
	\end{array}\right.
\end{equation}
The values $\{M_{\mathscr{S}}(w)\}_{w \in \Sigma^{*}}$ of $M_\mathscr{S}$ are the \emph{sub-Markov parameters} of $\mathscr{S}$.
From \cite{PetreczkyLPVSS} it then follows that two dLPV-SSAs have the same input-output behavior, if and only if
their sub-Markov functions are equal. 
%Moreover, the values of the sub-Markov function (sub-Markov parameters) can be
%determined from the input-output behavior.
%Sub-Markov parameters are analogous to Markov-parameters of linear systems, and just like in the linear case, a Ho-Kalman-like realization algorithm can be formulated which computes a dLPV-SSA from sub-Markov parameters \cite{PetreczkyLPVSS,RolandAbbas}. 
For a function $M:\Sigma^{*} \rightarrow \mathbb{R}^{n_\mathrm{y} \times n_\mathrm{u}}$, we will say that the dLPV-SSA $\mathscr{S}$ is a \emph{realization} of
$M$, if $M$ equals the sub-Markov function of $\mathscr{S}$, i.e., $M=M_{\mathscr{S}}$.
We will call two dLPV-SSAs input-output equivalent if they realize the same sub-Markov function.
For dLPV-SSA \eqref{eqn:LPV_SSA:det}, we call the integer $\nx$ the \emph{dimension} of $\mathscr{S}$.
We will call a dLPV-SSA \emph{minimal}, if there exists no other dLPV-SSA $\mathscr{S}^{'}$ with a smaller dimension and with the
same sub-Markov function.
%$\nx$ is larger than the dimension of $\mathscr{S}^{'}$ and their sub-Markov parameters are equal, i.e. $M_{\mathscr{S}}=M_{\mathscr{S}}^{'}$. 
We call a dLPV-SSA $\mathscr{S}$ a \emph{minimal  realization} of a function $M:\Sigma^{*} \rightarrow \mathbb{R}^{n_\mathrm{y} \times n_\mathrm{w}}$, if 
$\mathscr{S}$ is minimal and it is a realization of $M$. 
From \cite{PetreczkyLPVSS}, it follows that a dLPV-SSA is minimal if and only if it is span-reachable and observable, and the latter
properties are equivalent to rank conditions of the extended $n$-step reachability and observability matrices \cite[Definition 1, Theorem 2]{PetreczkyLPVSS}.
Furthermore, any dLPV-SSA  can be transformed to a minimal one  with the same sub-Markov function, using Kalman decomposition \cite[Corollary 1]{PetreczkyLPVSS}\footnote{\cite[Corollary 1]{PetreczkyLPVSS} should be applied with zero initial state}.
For a more detailed discussion see \cite{PetreczkyLPVSS}. %Note that by \cite{PetreczkyLPVSS}, minimal dLPV-SSAs %with the same sub-Markov functions are isomorphic: if
%$\mathscr{S}$ from \eqref{eqn:LPV_SSA:det} and
%$\mathscr{S}^{'}=(\{\mathcal{A}_{\sigma}^{'},\mathcal{B}_{\sigma}^{'}\}_{\sigma \in \Sigma},\mathcal{C}^{'},\mathcal{D}^{'})$ are both minimal dLPV-SSA and $M_{\mathscr{S}}=M_{\mathscr{S}^{'}}$, $\mathcal{D}=\mathcal{D}^{'}$, then, 
%there exists a non-singular matrix $\mathcal{T}$ such that $\mathcal{TA}_{\sigma}\mathcal{T}^{-1}=\mathcal{A}_{\sigma}^{'}$, $\mathcal{TB}_{\sigma}=\mathcal{B}_{\sigma}^{'}$ and $\mathcal{C}^{'}=\mathcal{CT}^{-1}$. 

==> Existence_and_minimality_of_an_asLPV-SSA_in_forward_innovation_form.tex <==
\section{Existence and minilality of asLPV-SSAs in innovation form}
\label{sect:min}
In this section we review the principal results on
existence and minimality of asLPV-SSA in innovation form. To this end, in  Subsection \ref{sect:real:red}  we recall from \cite{PetreczkyLPVSS} some results on realization theory of deterministic LPV-SSA. 
In Subsection \ref{sect:def:innov} we present the definition of asLPV-SSAs in innovation form, and
in Subsection \ref{subsect:min} we present results on existence and uniqueness of minimal asLPV-SSAs.
In Subsection \ref{Sect:algo} we present rank conditions for minimality of asLPV-SSAs and an algorithm for converting
any asLPV-SSA to a minimal one in innovation form. 
The results presented in this section follow from \cite{PetreczkyBilinear}, 
but they have never been formulated
%In contrast to \cite{PetreczkyBilinear}, we formulate the results below 
explicitly for LPV-SSAs. 

\input{Deterministic_LPV-SSA_representation}


\subsection{Definition of asLPV-SSA in innovation form}
\label{sect:def:innov}
Next, we  define what we mean by asLPV-SSA in innovation form.
%and we show that if $(\y,\p)$ has a realization by an asLPV-SSA, it has a minimal realization in innovation form. However, before we define a realization in innovation form,
To this end, we need to introduce the following notation for orthogonal projection.
\begin{Notation}[Orthogonal projection $E_l$]
	\label{hilbert:notation}
	Recall that the set of square integrable
	random variables taking values in $\mathbb{R}$, forms a Hilbert-space with the scalar product defined as $<\mathbf{z}_1,\mathbf{z}_2>=E[\mathbf{z}_1\mathbf{z}_2]$. We denote this Hilbert-space by $\mathcal{H}_1$. 
	Let $\mathbf{z}$ be a square integrable \emph{vector-valued} 
	random variable taking its values in $\mathbb{R}^k$.  Let $M$ be a closed subspace   of $\mathcal{H}_1$. 
	By the orthogonal projection of $\mathbf{z}$ onto the subspace $M$, \emph{denoted by $E_l[\mathbf{z} \mid M]$},
	we mean the vector-valued square-integrable random variable $\mathbf{z}^{*}=\begin{bmatrix} \mathbf{z}_1^{*},\ldots,\mathbf{z}_k^{*} \end{bmatrix}^T$ such that $\mathbf{z}_i^{*} \in M$ is the orthogonal projection of the $i$th coordinate $\mathbf{z}_i$ of $\mathbf{z}$ onto $M$, as it is usually defined for Hilbert spaces. 
	Let $\mathfrak{S}$ be a subset of square integrable random variables in $\mathbb{R}^p$ for some integer $p$, and 
	suppose that $M$ is generated by the coordinates of the elements of $\mathfrak{S}$, i.e. 
	$M$ is the smallest (with respect to set inclusion) closed subspace of $\mathcal{H}_1$
	which contains the set $\{ \alpha^Ts \mid  s \in \mathfrak{S}, \alpha \in \mathbb{R}^p\}$. 
	Then instead of $E_l[z \mid M]$ we use \( E_{l}[\mathbf{z} \mid \mathfrak{S}] \). %to denote the projection of $z$ to $M$.
	%Notice that $\mathbf{z}^{*}$ is uniquely determined by the following property: $E[(\mathbf{z}-\mathbf{z}^{*})\x^T]=0$ for all $\x \in Z$.
	% That is, $M$ is the smallest (with respect to set inclusion) closed linear subset such that for any $\mathbf{z}=(\mathbf{z}_1,\ldots,\mathbf{z}_p) \in Z$, $M$ contains the scalar random variables $\mathbf{z}_1,\ldots,\mathbf{z}_p$.
	%Notice also that one can interpret $E_{l}[\mathbf{z} \mid Z]$ as the best approximation (prediction) 
	%of $\mathbf{z}$ in terms of (infinite) linear combinations of elements~of~$Z$. 
\end{Notation}
This said, we define the \emph{innovation process $\eb$ of $\yb$ with respect to
$\p$} as follows:
	\begin{equation} 
		\label{decomp:lemma:innov2}
		\eb(t)=\yb(t)-E_l[\yb(t) \mid \{\z^{\yb}_w (t)\}_{w \in \Sigma^{+}}]
	\end{equation}
In other words, $\eb(t)$ is the difference between the output and its projection on its past values w.r.t. the scheduling process $\p$, i.e., $\eb$ is the best predictor of $\yb$ using the product of the output and scheduling past values from \eqref{eqn:zwu}.
\begin{Definition}[asLPV-SSA in innovation form]
    An asLPV-SSA of the form \eqref{eq:aslpv} is said to be in \emph{innovation form}, if it is a realization of $(\y,\p)$, $F=I_{\ny}$ and $\vb$ is the innovation process of $\yb$, i.e., $\vb = \eb$.
\end{Definition}
%In the sequel, we will need the following concept: $(\yb,\p)$ is full rank if for every $\sigma \in \Sigma$, the matrix $\expect{\eb(t)\eb^T(t)\p_\sigma^2(t)}$ is invertable. 


\subsection{Existence and uniqueness of minimal asLPV-SSA in innovation form}
\label{subsect:min}
Let  $\mathcal{S}$ %=(\{A_i,K_i,\}_{i=0}^{\pdim},C,I_{\ny},\eb)$ 
be an asLPV-SSA of the form \eqref{eq:aslpv} in innovation form with $F=I_{\ny}$.
%$,i.e., $\mathcal{S}$ is an asLPV-SSA of $(\yb,\p)$ in innovation form.
%(\{A_i,K_i,B_i\}_{i=0}^{\pdim},C,D,\eb^s)$ and  
Let $\widetilde{\mathcal{S}}=(\{\widetilde{A}_i,\widetilde{K}_i,\}_{i=0}^{\pdim},\widetilde{C},I_{\ny},\eb)$
be another asLPV-SSA of $(\yb,\p)$ in innovation form.
We say that $\mathcal{S}$ and $\widetilde{S}$ are \emph{isomorphic}, if there exists a non-singular matrix $T$ such that
$
\label{lemma:min1:eq1}
\widetilde{A}_i=TA_iT^{-1}, \widetilde{K}_i=TK_i, \widetilde{C}=CT^{-1}
$.

We will say that the process $(\yb,\p)$ is \emph{full rank}, if for all $i=1,\ldots, \pdim$, $Q_i=E[\eb(t)(\eb(t))^T\p_i^2(t)]$ is invertable. This is a direct extension of the classical notion of a full rank process. In the sequel, we will assume that $(\yb,\p)$ is full rank.

Furthermore, we will say
that $\yb$ is \emph{Square Integrable} process w.r.t. $\p$, 
abbreviated by \emph{SII}, if
it satisfies \cite[Definition 5]{PetreczkyBilinear}\footnote{with $\bu_{\sigma}=\p_{\sigma}$,
$\sigma \in \Sigma$ in the terminology of \cite{PetreczkyBilinear}}.
For the convenience of the reader, the definition of an SII process is presented in Appendix \ref{App:def}, Definition \ref{Defn:SII}. From \cite[Remark 2]{PetreczkyBilinear} it follows that if $(\yb,\p)$ has a realization by an asLPV-SSA and $\p$ is bounded, then $\yb$ is SII.
\begin{Theorem}[Existence and uniqueness]
\label{theo:min}
Assume that $(\yb,\p)$ has an asLPV-SSA  realization and that $\yb$ is full rank and SII w.r.t. $\p$.
It follows that:	
\begin{enumerate}
\item
\label{theo:min:1}
$(\y,\p)$ has a minimal asLPV-SSA realization in innovation form
\item
\label{theo:min:2}
Any two minimal asLPV-SSA realizations of $(\yb,\p)$ in innovation form are isomorphic.  
\end{enumerate}
\end{Theorem}

The proof of this theorem follows \cite[Theorem 2]{PetreczkyBilinear} by
using the correspendence between \GBS\ and asLPV-SSA. 
%in the terminology of \cite{PetreczkyBilinear}, an asLPV-SSA corresponds to a stationary generalized bilinear system w.r.t. $\p$.

Theorem \ref{theo:min} implies that asLPV-SSAs in innovation form have the useful property that, when they are minimal, they are unique up to isomorphism, and
assuming that the asLPV-SSA which generates the data is minimal does not restrict the class of 
possible output.
That is, for system identification it is preferable to consider parametrizing the elements of minimal asLPV-SSAs in innovation form. This motivates finding conditions for an asLPV-SSA to be minimal in innovation form and formulating algorithms for transforming an asLPV-SSA to a minimal one
in innovation form.  To this end, in Subsection \ref{Sect:algo} we present a rank condition 
for minimality and a minimization algorithm based on the results of \cite{PetreczkyBilinear}. 
However, the results of Subsection \ref{Sect:algo} do not allow checking that an asLPV-SSA is in innovation form.
Moreover, the algebraic conditions for minimality are difficult to apply.
%Moreover, the rank conditions and the minimization algorithms require
%the solution of a Lyapunov-style equality which makes the difficult to apply to parametrizations. 
Motivated by this, in Section \ref{sect:main} we present more user-friendly 
characterizations of minimality and being in innovation form.


%\subsection{Conditions for minimality of asLPV-SSA, minimization and realization algorithms}
%  Minimality of asLPV-SSAs can be partially characterized via rank conditions, similar to
%  rank conditions for deterministic LPV-SSA. Moreover, it is possible to formulate an 
%  algorithm for transforming an asLPV-SSA to a minimal one in innovation form. 
  
 \subsection{Rank conditions and minimization algorithm}
 %for transforming a asLPV-SSA to minimal asLPV-SSA in innovation form}
\label{Sect:algo}
%To be able to obtain an asLPV-SSA representation in the forwrad innovation form, we present a reliable algorithm defined in the following definitions, where we associate a dLPV-SSA with the original asLPV-SSA and, afterwards, using the later dLPV-SSA, we associate with it the asLPV-SSA in innovation form.
%\begin{Definition}[dLPV-SSA associated with asLPV-SSA]\label{defn:det_asco_stationary}
In order to present the rank conditions for minimality of asLPV-SSA and the minimization algorithm, we need
to define the \emph{dLPV-SSA associated with asLPV-SSA} as
$$\mathscr{S}_{\mathcal{S}}=(\{\sqrt{p_i} A_i,\Bs_i\}_{i=1}^{\pdim},C,I_{\ny}), $$
where  %$\{\Bs_i\}_{i=1}^{\pdim}$ %are expressed as follows:
\begin{equation}
\label{min:eq-1}
\Bs_i=\frac{1}{\sqrt{p_i}}(A_iP_iC^T + K_iQ_iF^T)
\end{equation}
and  $Q_i=E[\vb(t)\vb^T(t)\p_i^2(t)]$ for $i=1,\ldots,\pdim$, 
and $\{P_i\}_{i=1}^{\pdim}$ are the computed as follows:
%\begin{Remark}[Computing $\Bs_i$]
%\label{gi:comp}
% In order to compute  $\{P_i\}_{i=1}^{\pdim}$ and hence $\{\Bs_i\}_{i=1}^{\pdim}$, we can use
%\cite[Lemma 5]{PetreczkyBilinear}, which states:
 %\begin{equation}
%\label{gi:comp:eq}
 \(    P_i = \lim_{\mathcal{I} \rightarrow \infty} P_i^{\mathcal{I}} \),
 %\end{equation}
 and $\{P_i^\mathcal{I}\}_{i=1}^{\pdim}$ satisfy the following recursions:
\begin{equation}
\label{gi:comp:eq1}
    P_i^{\mathcal{I}+1}=p_{i} \sum_{j=0}^{\pdim} (A_jP_j^{\mathcal{I}}A_j^T + K_jQ_jK_j^T)
\end{equation}
with $P_i^0 = \mathbf{O}_{n_x,n_x}$ where $\mathbf{O}_{n_x,n_x}$ denotes the $n_x \times n_x$ matrix with all zero entries.
  %In particular, $P_i=p_{i} \sum_{j=0}^{\pdim} (A_jP_jA_j^T + K_jQ_jK_j^T)$ . 
%\end{Remark}
%\end{Definition}
Note that the existence of the limit of $P_i^\mathcal{I}$ when $\mathcal{I}$ goes to infinity follows from \cite[Lemma 5]{PetreczkyBilinear}.
%We will call \eqref{eq:aslpv} \emph{span-reachable} and \emph{observable}, if the associated 
%dLPV-SSA $\mathscr{S}_{\mathcal{S}}$ is span-reachable, respectively observable.
From \cite{PetreczkyBilinear} it also follows that
the dLPV-SSA associated with an asLPV-SSA $\mathscr{S}$ represents a realization of Markov-function
$\covseq: \Sigma^{*} \rightarrow \mathbb{R}^{\ny \times \ny}$, 
$$\covseq(w) =\left\{ \begin{array}{ll} E[\yb(t) (\zwy(t))^{T} ] & w \in \Sigma^{+}\\
I_{\ny} & w=\epsilon \\ \end{array}\right.$$ 
computed from the covariances of $\y$.

Then from \cite{PetreczkyBilinear} we can derive the following.
\begin{Theorem}[Rank conditions]
\label{theo:rank_cond}
 An asLPV-SSA is a minimal realization of $(\y,\p)$, if and only if the associated dLPV-SSA is minimal.
\end{Theorem}
The proof follows from the proof of Theorem 2 of \cite{PetreczkyBilinear} by noticing that the recognizable representation associated with a GBS in the terminology of \cite{PetreczkyBilinear} corresponds to the dLPV-SSA associated with an asLPV-SSA in the terminology of this paper.
%Note that asLPV-SSA corresponds to GBS in the terminology of \cite{PetreczkyBilinear}.
From \cite{PetreczkyLPVSS} it follows that minimality of the associated dLPV-SSA can be checked using rank
conditions for the corresponding extended reachability and observability matrices. 
Note, however, that minimal asLPV-SSAs, realizing the same output, may not be isomorphic. In fact, in Section \ref{sect:examp}, Example \ref{sim:examp} presents a counter-example. 

%We can not only associate a dLPV-SSA  with an asLPV-SSA which realizes the sequence $\covseq$, 
Vice versa, with any
dLPV-SSA realization of $\covseq$ we can associate an asLPV-SSA in innovation form. This latter relationship
is useful for formulating a minimization algorithm. 
%\begin{Definition}[asLPV-SSA associated with dLPV-SSA]\label{defn:det_asco_stationary}
More precisely, consider a dLPV-SSA 
$$\mathscr{S}=(\{\hat{A}_i, \hat{G}_i\}_{i=1}^{\pdim}, \hat{C}, I_{\ny})$$
which is a minimal realization
of $\covseq$. 
%$\sum_{i=1}^{\pdim} \hat{A}_i \otimes \hat{A}_i$ is stable,
Define the \emph{asLPV-SSA $\mathcal{S}_{\mathscr{S}}$ associated with $\mathscr{S}$} as 
$$ \mathcal{S}_{\mathscr{S}}=(\{\frac{1}{\sqrt{p_i}} \hat{A}_i, \hat{K}_i\}_{i=1}^{\pdim},\hat{C},I_{\ny},\eb), $$
where $\hat{K}_i=\lim_{\mathcal{I} \rightarrow \infty} \hat{K}_i^{\mathcal{I}}$, and
	%\begin{equation*}
	   %\hat{A}^{s}_{\sigma}=\frac{1}{\sqrt{p_{\sigma}}} \hat{A}_{\sigma}, ~ 
       %$$\hat{K}_{\sigma}=\lim_{i \rightarrow \infty} \hat{K}_{\sigma}^{\mathcal{I}}$$
	%\end{equation*} 
	$\{\hat{K}_{\sigma}^{\mathcal{I}} \}_{\sigma \in \Sigma, \mathcal{I} \in \mathbb{N}}$ satisfies the following recursion
	\begin{equation}
		\label{statecov:iter}
		\begin{split}
			%\hat{P}^{i+1}_{\sigma} \!&=\! \sum \limits_{\sigma_{1} \in \Sigma, \sigma_{1} \sigma \notin L } \psig \left( \hat{A}_{\sigma_{1}} \hat{P}^{i}_{\sigma_{1} }  \hat{A}^{T}_{\sigma_{1}}  + \hat{K}_{\sigma_{1}} \hat{Q}^{i}_{\sigma_{1} }  \hat{K}^{\mathcal{I}})^{T}_{\sigma_{1}}  \right)\\
			& 	\hat{P}^{\mathcal{I}+1}_{\sigma} = \sum \limits_{\sigma_{1} \in \Sigma} \psig \left(\frac{1}{p_{\sigma_1}} 
			\hat{A}_{\sigma_{1}} \hat{P}^{\mathcal{I}}_{\sigma_{1} }  (\hat{A}_{\sigma_{1}})^{T}  + \hat{K}_{\sigma_{1}}^{\mathcal{I}} \hat{Q}^{\mathcal{I}}_{\sigma_{1} }  (\hat{K}^{\mathcal{I}}_{\sigma_{1}})^T  \right)\\
			& \hat{Q}^{\mathcal{I}}_{\sigma} = \psig T_{\sigma,\sigma}^{y} - \hat{C}  \hat{P}^{\mathcal{I}}_{\sigma } (\hat{C})^{T}  \\ 
			& \hat{K}^{\mathcal{I}}_{\sigma} = \left( \hat{\Bs}_{\sigma} \sqrt{\psig} - \frac{1}{\sqrt{\psig}}
			\hat{A}_{\sigma} \hat{P}^{\mathcal{I}}_{\sigma}  (\hat{C})^{T} \right) \left(  \hat{Q}^{\mathcal{I}}_{\sigma} \right)^{-1}
		\end{split}
	\end{equation}
	where $\hat{P}^{0}_{\sigma} = \mathbf{O}_{n_x,n_x}$ and $T_{\sigma,\sigma}^{y} = \expect{\y(t) (\zwy(t))^{T}}$. 
%Intuitively, the limit of the matrices \eqref{statecov:iter}
%µsolve an extension of the well-known algebraic Riccati equation,
%see \cite[Remark 7]{PetreczkyBilinear}.
%\end{Definition}
 %\begin{Lemma}
%\label{min:col}
From \cite{PetreczkyBilinear} it follows that
%If $\mathcal{S}$ is an asLPV-SSA representation of $(\yb,\p)$, then the associated dLPV-SSA $\mathscr{S}_{\mathcal{S}}$ is a %realization of $M_{\yb}$, where $M_{\yb}$ is the Markov-parameters which is equal to the following covariance matrix:
%\begin{equation}\label{eqn:covseq}
%	M_\y = \covseq(w) = %\left\{\begin{array}{rl}
%	E[\yb(t) (\zwy(t))^{T} ]  %& w \in \Sigma^{+} \\
%	%I_{\ny} &  w=\epsilon 
	%             \end{array}\right. 
%\end{equation}
%Conversely, if $(\yb,\p)$ has an asLPV-SSA, and 
if $\mathscr{S}$ is a minimal dLPV-SSA realization of $\covseq$, and $(\yb,\p)$ is full rank, then the associated asLPV-SSA $\mathcal{S}_{\mathscr{S}}$ is an asLPV-SSA of $(\yb,\p)$. 
%\end{Lemma}
%We will call \eqref{eq:aslpv} \emph{span-reachable} and \emph{observable}, if the associated 
%dLPV-SSA $\mathscr{S}_{\mathcal{S}}$ is span-reachable, respectively observable.
%the extended $\nx-1$-step reachability and observability matrices of $\mathscr{S}_{\mathcal{S}}$ satisfy $\rank \mathcal{R}_{\nx-1}=\nx$ and $\rank \mathcal{O}_{\nx-1}$.
%We will say that an asLPV-SSA of the form \eqref{eq:aslpv} is in innovation form, if the noise process $\vb$ equals the innovation process $\eb$ from  
%\eqref{decomp:lemma:innov2}. Note that the asLPV-SSA associated with a dLPV-SSA is in %innovation form. 

The discussion above suggests the following realization algorithm
for transforming an asLPV-SSA $\mathcal{S}$ to a minimal one, which can be deduced from \cite{PetreczkyBilinear}.
\begin{algorithm}[h!]

\caption{Minimization algorithm
\label{alg:min}}
~~\textbf{Input :} The asLPV-SSA $\mathcal{S} =(\{A_{\sigma},K_{\sigma}\}_{\sigma=1}^{\pdim},C,F,\vb)$.
\hrule\vspace*{.1cm}
\begin{enumerate}
    \item  Compute the dLPV-SSA $\mathscr{S}_{\mathcal{S}}$ associated with $\mathcal{S}$ and compute $T_{\sigma,\sigma}^{\y} = \frac{1}{\psig}(C\Psig C^{T} + F\Qsig F^T)$ and $Q_\sigma=E[\vb(t)\vb^T(t)\p_\sigma^2(t)]$
           	%Note that, as a consequence for  $\mathcal{S}_{\mathscr{S}}$ being an asLPV-SSA representation of $(\y,\p)$ of the %form \eqref{eq:aslpv}, we can expressed the covariance as:

    \item Transform  the dLPV-SSA $\mathscr{S}_{\mathcal{S}}$ to
    a minimal dLPV-SSA 
    $\mathscr{S}_m$ using \cite[Corollary 1]{PetreczkyLPVSS}.
    
    \item Construct the asLPV-SSA $\mathcal{S}_{{\mathscr{S}}_m}$
    associated with $\mathscr{S}_m$.
\end{enumerate}
\hrule\vspace*{.1cm}
\textbf{Output :} The asLPV-SSA $\mathcal{S}_{{\mathscr{S}}_m}$.
%in \eqref{gi:comp:eq}
%(for computing $\mathscr{S}_{\mathcal{S}}$) and 
% \eqref{statecov:iter} (for computing $\mathcal{S}_{\mathscr{S}}$)  the usual numerical solutions are used to
%approximate limits of converging sequences.
\end{algorithm}

From \cite[Theorem 3]{PetreczkyBilinear}, it follows that Algorithm \ref{alg:min} returns a minimal realization of $(\yb,\p)$, if $\mathcal{S}$ is an asLPV-SSA realization of $(\yb,\p)$ in innovation form. Note that Algorithm \ref{alg:min} requires only the knowledge of the matrices of $\mathcal{S}$ and the noise covariance matrices $Q_\sigma$. Also note that all the steps above are computationally efficient, however, they require finding the limits
of $P_{\sigma}^{\mathcal{I}}$ and $\hat{K}_{\sigma}^{\mathcal{I}}$ for $\mathcal{I} \rightarrow \infty$ respectively. 
Also note that, in \cite{MejariCDC2019}, it exists another minimization algorithm which uses covariances matrices.
\begin{Remark}[Challenges]
\label{rem:motiv1}
The main disadvantage of  
verifying the rank condition of Theorem \ref{theo:rank_cond} or applying Algorithm \ref{alg:min} is the necessity of constructing a dLPV-SSA and 
the necessity to find the limit of the matrices in
\eqref{statecov:iter}. The latter represents an extension of
algebraic Riccati equations \cite[Remark 7]{PetreczkyBilinear} and even for
the linear case requires attention. Moreover, the rank
conditions of Theorem \ref{theo:rank_cond} are not easy to apply to
parametrizations: even if the dependence of the matrices $\{A_i,K_i\}_{i=1}^{\pdim}$
and $C$ on a parameter $\theta$ are linear or polynomial, the dependence of
the matrices of the associated dLPV-SSA need not remain linear or polynomial,
due to the definition of $\Bs_i$ in \eqref{min:eq-1}. For the same reason,
it is difficult to analyze the result of 
applying Algorithm \ref{alg:min} to elements of a parametrization.
Moreover, the
conditions of Theorem \ref{theo:rank_cond} do not allow us to check if
the elements of a parametrizations are in innovation form. 
These shortcomings motivate the contribution of Section \ref{sect:main}.
\end{Remark}
%Therefore, in the following section we propose new conditions for an asLPV-SSA in innovation form.



 %In  this section, we present an algebraic conditions, in order to verify the existence of a realization in innovation form. %To this end, in Subsection \ref{sect:real:red} we recall the definition of a deterministic LPV-SSA representation, before presenting the main conditions in Subsection \ref{sect:main:cond}. 







==> Stationary_LPV-SSA_representation.tex <==
\subsection{Stationary LSS representation and notation}
\label{Subsec:assumptions3}
After identifying the necessary process properties and notations, we are now ready to present the definition of the \emph{stationary LSS}.
\begin{Definition}[Stationary sLSS]
\label{defn:LPV_SSA_wo_u}
\label{def:Stationary}
 %The  GLSS 
  A  \emph{stationary LSS} (abbreviated 
  sLSS) of $(\y,\bu,\p)$ is a system \eqref{eq:aslpv}, such that
%a process $\r$ taking values in $\mathbb{R}^{p}$, 
%is a system of the form \begin{equation}
%	\label{eq:aslpv}
%            \mathcal{S} \left\{     \begin{aligned}
%                 &  \tilde{\xb}(t+1)=\sum_{i=1}^{\pdim} (\tilde{A}_i\tilde{\xb}(t)+\tilde{K}_i\tilde{\vb}(t))\p_i(t) \\
%                 & \r(t)=\tilde{C}\tilde{\xb}(t)+\tilde{F}\tilde{\vb}(t)
%		\end{aligned}\right.
%               \end{equation}
%           where 
%	$\tilde{A}_{\sigma} \in \mathbb{R}^{\tilde{n} \times \tilde{n}}, \tilde{K}_{\sigma} \in \mathbb{R}^{\tilde{n} \times \tilde{m}}$,
%	$\tilde{C} \in \mathbb{R}^{p \times \tilde{n}}$, $\hat{F} \in \mathbb{R}^{p \times \tilde{m}}$, 
%        and $\vb$ is a process taking values in $\mathbb{R}^{\tilde{m}}$, 
%         and the following holds:
\begin{itemize}
	
		
	\item[\textbf{1.}]
		$\mathbf{w}=\begin{bmatrix} \vb^T, \!\! & \!\! \bu^T \end{bmatrix}^T$ is a white noise process w.r.t. $\p$. 

    \item[\textbf{2.}]
  The process
  $\begin{bmatrix} \xb^T\!\!, & \!\! \mathbf{w}^T \end{bmatrix}^T$  is a ZMWSSI, and 
     $    
        %\forall (\sigma,w )\in \Sigma \times \Sigma^{+}:
        E[\z^{\xb}_{\sigma}(t)(\z^{\mathbf{w}}_{\sigma}(t))^T]=0, ~
        E[\xb(t)(\z^{\mathbf{w}}_w(t))^T]=0,
    $
  for all $\sigSet$, $w \in \Sigma^{+}$.
  
  
  % and $E[\tilde{\vb}(t)\tilde{\vb}^T(t)\p_i^2]=Q_i$.
	
	\item[\textbf{3.}]
		The eigenvalues of the matrix $\sum_{\sigSet} \psig {A}_{\sigma} \otimes {A}_{\sigma}$ are inside the open unit circle.

    \item[\textbf{4.}]  For all $\sigma_1,\sigma_2 \in \Sigma$, if $(\sigma_1,\sigma_2) \notin \mathcal{E}$, then
  $A_{\sigma_2}A_{\sigma_1}=0$ and $A_{\sigma_2}\begin{bmatrix} B_{\sigma_1} & K_{\sigma_1} \end{bmatrix}E[\z^{\mathbf{w}}_{\sigma_1}(t) (\z_{\sigma_1}^{\mathbf{w}}(t))^T]=0$.

		%	\end{enumerate} 
	%We call $\tilde{\xb}$ the state process and $\tilde{\vb}$ the noise process. 
       %We say that a asLPV-SSA is a realization of a process $\tilde{\r}$, if its output process equals $\r$. 
       \end{itemize}
If $B_i=0$, $i \in \Sigma$, and $D=0$  the we call \eqref{eqn:LPV_SSA} an \emph{autonomous stationary} GLSS (asGLSS) of $(\y,\p)$.
%       (abbreviated as \emph{asGLSS of $(\y,\p)$}).
\end{Definition}
%Note that, condition \textbf{(2)} implies that $\Tilde{\vb}$ is a white noise, i.e., $E[\Tilde{\vb}(t)]=0$ and $E[\Tilde{\vb}(t)\Tilde{\vb}^T(s)]=0$ for $t \neq s$.

%In the terminology of \cite{PetreczkyBilinear}, an asLPV-SSA corresponds to a stationary \GBS\  w.r.t. inputs $\{\p_{\sigma}\}_{\sigma \in \Sigma}$. 
%From \cite{PetreczkyBilinear}, if a process $\r$ can be represented by an asLPV-SSA, then $\r$ is a ZMWSSI process and 
%$\xb$ is uniquely determined by $\vb$ and the matrices $( %\{A_{\sigma},K_{\sigma}\}_{\sigma \in \Sigma}, C,D)$. 
Note that the processes $\xb$ and $\yb$ are ZMWSII, in particular, they
are wide-sense stationary, and that $\xb$ is orthogonal to the future values of the process $\mathbf{w}$.
We should mention that we concentrate on wide-sense stationary processes, because it is difficult to estimate the distribution of non-stationary processes. Also, wide-sense stationary processes solve the problem of the initial state conditions.

It can be shown that the state of a sLSS,
is uniquely determined by the matrices of the sLSS and the process $\mathbf{w}=\begin{bmatrix} \ub^T & \vb^T
\end{bmatrix}^T$. To this end, we introduce the following notation.
%In order to define this notion more precisely, 
\begin{Notation}[Matrix Product]\label{not:product}
	Consider $n \times n$ square matrices $\{A_{\sigma}\}_{\sigSet}$. For any word $\wordSet{+}$ of the form $w = \sigma_{1}\sigma_{2}\cdots\sigma_{k}$, $k\!>\!0$ and $\sigma_{1}, \ldots, \sigma_{k} \in \Sigma$, we define 
	%\begin{equation*}
	$$A_{w} = A_{\sigma_{k}}A_{\sigma_{k-1}}\cdots A_{\sigma_{1}}$$
	%\end{equation*}
	%	For example, $w = 123$, $A_{w} = A_{123} = A_{3}A_{2}A_{1}$.
	For an empty word $\epsilon$, let $A_{\epsilon} = I_n$.
\end{Notation}
From \cite[Lemma 2]{PetreczkyBilinear} it follows that
% From \cite{PetreczkyBilinear}, it follows that
\begin{equation*}
	%\label{stat:state:eq1}
	%\begin{split}
	 \xb(t)=\sum_{v \in \Sigma^{*},\sigma \in \Sigma}
	   \sqrt{p_{\sigma v}} A_{v}K_{\sigma}\z^{\vb}_{\sigma v}(t)
	%
	%\sum_{\sigma_0 \in \Sigma} \sqrt{p_{\sigma_0}} K_{\sigma_0}\z^{\vb}_{\sigma_0}(t) +   
	\\ 
	%& \sum_{k=1}^{\infty} \sum_{\sigma_0,\sigma_1,\ldots, \sigma_k \in \Sigma} 
	% \sqrt{p_{\sigma_0\sigma_1 \cdots \sigma_k}}  A_{\sigma_k}A_{\sigma_{k-1}} \cdots A_{\sigma_1}K_{\sigma_0}\z^{\vb}_{\sigma_0 \cdots \sigma_k}(t) 
	% \end{split}
\end{equation*}
where the infinite sum on the right-hand side is  absolutely convergent in the mean square sense.
This prompts us to use the following notation.
\begin{Notation}
       We identify the sLSS $\mathcal{S}$ of the form \eqref{eq:aslpv} with the tuple 
       $\mathcal{S} =(\{A_{\sigma},B_{\sigma},K_{\sigma}\}_{\sigma=1}^{\pdim},C,D,F,\vb,\ub,\p)$. When $\p$ and $\ub$ are clear from the context, we use the notation $\mathcal{S} =(\{A_{\sigma},B_{\sigma},K_{\sigma}\}_{\sigma=1}^{\pdim},C,D,F,\vb)$.
\end{Notation}

Finally, we need to define what we mean by an sLSS realization of a process.
An sLSS $\mathcal{S}$ of the form \eqref{eq:aslpv} is a \emph{realization of
a pair $(\tilde{\y},\tilde{\p})$}, if $\tilde{\y}=\y$, $\tilde{\p}=\p$. 
If $\mathcal{S}$ is of the form \eqref{eq:aslpv}, then we 
call the state-space dimension $\nx$ the \emph{dimension} of $\mathcal{S}$ and we denote it by
$\dim \mathcal{S}$.
We say that the asLPV-SSA $\mathcal{S}$ is a \emph{minimal} realization of $(\tilde{\y},\tilde{\p})$, if for any asLPV-SSA realization $\mathcal{S}^{'}$ of
$(\tilde{\y},\tilde{\p})$, the dimension of $\mathcal{S}^{'}$ is not smaller than $\dim \mathcal{S}$.





==> Technical_assumptions_on_the_scheduling_process.tex <==
\section{Preliminaries}
\label{sect:prelim}
%We will present some technical notations and definitions regarding the involved processes, in order to help prepare the exposition of the main results.
In the sequel, we will use the standard terminology of probability theory \cite{Bilingsley}. In particular, all the random variables and stochastic processes are understood w.r.t. to a fixed probability space $\left(\Omega, \mathcal{F}, \mathcal{P}\right)$, where $\mathcal{F}$ is a $\sigma$-algebra over the sample space $\Omega$.
	%(\emph{i.e.}, $\mathcal{F}$ is a collection of subsets of $\Omega$, that includes $\Omega$ itself, is closed under complement, is closed under countable unions and is closed under countable intersections) and $\mathcal{P}$ is a probability measure on $\mathcal{F}$. For two $\sigma$-algebras $\mathcal{F}_i$, $i=1,2$, $\mathcal{F}_1 \lor \mathcal{F}_2$ denotes the smallest $\sigma$-algebra generated by the $\sigma$-algebras $\mathcal{F}_1,\mathcal{F}_2$. 
The expected value of a random variable $\mathbf{h}$ is denoted by $E[\mathbf{h}]$ and conditional expectation w.r.t. $\sigma$- algebra $\mathcal{F}$ is denoted by $\expect{\mathbf{h} \mid \mathcal{F}}$. 
All the stochastic processes in this paper are discrete-time ones defined over the time-axis $\mathbb{Z}$ of the set of integers:
a stochastic process $\r$ is a collection of random variables
$\{\r(t)\}_{t \in \mathbb{Z}}$ taking values in some set $X$. 
Note that we use bold letters to denote random variables and stochastic processes.

Next, we define the class of systems studied in this paper. A \emph{Linear Switched System} (LSS) is a system described by the following state-space representation:
 \begin{equation}
	\label{eq:aslpv}
            \mathcal{S} \left\{     \begin{aligned}
                 &  \xb(t+1)=\sum_{i=1}^{\pdim} (A_i\xb(t)+B_i\ub(t)+K_i\vb(t))\p_i(t) \\
                 & \y(t)=C\xb(t)+D\ub(t)+F\vb(t)
		\end{aligned}\right.
               \end{equation}
           where 
	$A_{i} \in \mathbb{R}^{n \times n}, K_{i} \in \mathbb{R}^{n \times m}$,
	$C \in \mathbb{R}^{p \times n}$, $F \in \mathbb{R}^{n_y \times m}$,
	and $\xb$ is the state process, $\vb$ is the noise process and $\y$ is the output process. Also, $\p=\begin{bmatrix} \p_1,\ldots,\p_{\pdim} \end{bmatrix}^T$ is the 
	switching process and $\p \in \begin{Bmatrix} b_i \end{Bmatrix}_{i=1}^{\pdim}$, where $b_i = \begin{bmatrix} 0, \ldots, 0,1,0, \ldots, 0 \end{bmatrix}$ is the $\pdim$-tuple with all components equal to 0, except the \emph{i}th, which is 1. Then, the switching process can be represented as follows:
 $$\p_{i}(t)=\chi(\btheta(t)=i)=
  \begin{cases}
  1 & \text{if $\btheta(t)=i,$}\\ 
  0 & \text{otherwise.}
  \end{cases}$$ for all $i \in \{1, \ldots, \pdim\}$, $t \in \mathbb{Z}$. 
   We will handle in this paper two cases: \textbf{case(1)} where the process $\btheta$ is an i.i.d. process, \textbf{case(2)} where $\btheta$ is a Markov process.
	
	
	Note that all the involved processes are defined for both negative and positive time. This may create technical problems for
	the existence of a solution and the role of initial state. 
	In this paper we will circumvent this problem by considering
	LSS which are mean-square stable in a suitable sense and
	state process of which is stationary. 
 %In order to define this class of LSS we will have to recall from \cite{PetreczkyBilinear} some notation and terminology. 
	
	

%A discrete-time stochastic process is a collection $\{\mathbf{r}(t)\}_{t \in \mathbb{Z}}$ taking values in $X$, where $\mathbf{r}(t) \in X$ is a random variable for all $t \in \mathbb{Z}$. Let $\mathbf{x}$ be a stochastic process taking values in $\mathbb{R}^{n}$; $\mathbf{x}$ is called \emph{zero mean}, if $\expect{\mathbf{x}(t)} = 0$ for all $t \in \mathbb{Z}$; $\mathbf{x}$  is called \emph{square integrable}, if the expectations $\expect{\mathbf{x}(t)}$, $\expect{\xb(t) \xb^{T}(t)}$ exist for all $t \in \mathbb{Z}$. A square-integrable process $\xb$ is called \emph{wide sense stationary}, if for every $s, t, k \in \mathbb{Z}$, the value of the expectations $\expect{\xb(t+k)\xb^{T}(s+k)}$ and $\expect{\xb(t+k)}$ is independent of $k$.
%We denote the $n \times n$ identity matrix by $I_n$.
	

 	
	

\subsection{Properties of the input and output processes}
\label{Subsec:assumptions1}
 Below we define the concept of 
 %admissible input processes and 
 ZMWSII processes w.r.t. switching process. These concepts will be used to define the nature of the processes and the subclass of the LSSs we will work with. 
 %assume that the scheduling process $\p$ is an admissible process in the terminology of \cite{PetreczkyBilinear}.
 To this end, we will need the following notation from automata theory which will be used for other 
 purposes too
\begin{Notation}[Sequences over $\Sigma$]
	Consider the finite set
	\[ \Sigma = \{1, \ldots, \pdim\}. \]%and letter $\sigSet$ will denote an integer. 
%\end{Notation}
A \emph{non empty word} over $\Sigma$ is a finite sequence of letters, i.e., $w = \sigma_{1}\sigma_{2}\cdots \sigma_{k}$, where $0 < k \in \mathbb{Z}$, $\sigma_{1}, \sigma_{2}, \ldots, \sigma_{k} \in \Sigma$. The set of \emph{all} nonempty words is denoted by $\Sigma^{+}$. We denote an \emph{empty word} by $\epsilon$. Let $\Sigma^{*} = \epsilon \cup \Sigma^{+}$. The concatenation of two nonempty words $v = a_{1}a_{2}\cdots a_{m}$ and  $w= b_{1}b_{2}\cdots b_{n}$ is defined as $vw = a_{1}\cdots a_{m} b_{1} \cdots b_{n}$ for some $m,n > 0$. Note that if $w = \epsilon$ or $v= \epsilon$,  then $v\epsilon = v$ and $\epsilon w = w$, moreover, $\epsilon \epsilon = \epsilon$. The length of the word $w \in \Sigma^{*}$ is denoted by $|w|$, and $|\epsilon| =0$. 
\end{Notation}
%\begin{Example*}
%	For $\pdim=2$,  $\Sigma = \{1,2\}$, $\Sigma^{*}= \{\epsilon,1,2,11,12,21,22,111, \ldots\}$, for the word $w=111 \in \Sigma^{*}$, $|w|=3$.
%\end{Example*}
%Below we will state a number of technical assumptions. We will start by stating some assumptions on the scheduling process $\p$. More precisely, we will have to impose assumptions on the product of the scheduling variables. To this end, we define the following notation.

With the notation above, we can identify the process $\p$ with the collection 
$\{\p_{\sigma}\}_{\sigma \in \Sigma}$ of its components. 
%In this paper we will deal with the following type of switching process: 
%We will say that $\p$ is an \emph{admissible scheduling process}, if the collection
%$\{\p_{\sigma}\}_{\sigma \in \Sigma}$ is an admissible collection of input processes in the sense of
%\cite[Definition 1]{PetreczkyBilinear} for $S=\Sigma \times \Sigma$. For the convenience of the reader, a version of \cite[Definition 1]{PetreczkyBilinear} is presented in Appendix \ref{App:def}.
%Before proceeding further we will present examples of admissible scheduling sequences.
%\begin{Example}[White noise  scheduling]
%\label{i.i.d. input}
 %The scheduling process $\p = [\p_1, \p_{2}, \ldots, \p_{\pdim}]^{T}$ is independent identically distributed (i.i.d.) such that
 %for all $i,j=2,\ldots, \pdim$, $t \in \mathbb{Z}$, $\p_i(t), \p_j(t)$ are independent and
%$\p_i(t)$ is zero mean, then $\p$ is admissible. %In this case, $\p$ is a admissible scheduling process %$p_{\sigma}=E[\p_{\sigma}^2(t)]$. 
% It to see that 
% for all $t \in \mathbb{Z}$, we have $\uw{1}(t) \equiv 1$, and for each $\sigma =2, \ldots, \pdim$, $\uw{\sigma}$ is zero-mean, and $p_1=1$ and $\pi_i=
% independent identically distributed (i.i.d.) process.
 %\end{Example}
% \begin{Notation}[Discrete valued process]
 %\label{disc:input}
%  Assume that there exists a process $\btheta$
%  which takes its values from a finite set $\Sigma=\{1,\ldots,\pdim\}$.  Let $$\p_{\sigma}(t)=\chi(\btheta(t)=\sigma)=
%  \begin{cases}
%  1 & \text{if $\btheta(t)=\sigma,$}\\ 
%  0 & \text{otherwise.}
%  \end{cases}$$ for all $\sigma \in \Sigma$, $t \in \mathbb{Z}$. %Let $S=\Sigma \times \Sigma$, $L=\Sigma^{+}$ and  
  %$p_{\sigma}=P(\btheta(t)=\sigma)$, $\alpha_{\sigma}=1$ for all $\sigma \in \Sigma$.
%  Then $\p(t)=\begin{bmatrix} \p_1(t) & \ldots & \p_{n_{\mathrm p}} \end{bmatrix}^T$ is the switching pocess. 
% \end{Notation}
% We will handle in this paper two cases: \textbf{case(1)} where the process $\btheta$ is an i.i.d. process, \textbf{case(2)} where $\btheta$ is a Markov process.
% For further examples, see \cite{PetreczkyBilinear}. 
 
 %We assume that the scheduling process $\p$ is admissible throughout the paper. 

Furthermore, we will use the definition of a \emph{Zero Mean Wide Sense Stationary (abbreviated by  ZMWSII) process with respect to $\p$} from \cite[Definition 2]{PetreczkyBilinear}.
%Similarly, we will say that 
%$\r$ is \emph{square integrable  (abbreviated by SII) with respect to $\p$}, if
%$\r$ is SII w.r.t. $\{\p_{\sigma}\}_{\sigma \in \Sigma}$
%according to \cite[Definition 5]{PetreczkyBilinear}.
%In addition to the assumptions on the scheduling process, we present assumptions on the input and output processes w.r.t. the scheduling process $\p$. First, it is necessary to mention that the
For the convenience of the reader this definition is reformulated in Appendix \ref{App:def} as Definition \ref{def:ZMWSSI}.
%and Definition \ref{Defn:SII} of 
%Appendix \ref{App:def}.

In order to explain the intuition behind these definitions, 
and because we will use them later on,
we define the following products of scheduling variables along a sequence from $\Sigma^{+}$.
For every word $\wordSet{+}$ where $w=\word$, $k \geq 1$, $\sigma_{1},\ldots, \sigma_{k} \in \Sigma$, we define the  process $\uw{w}$ as follows:
%the scalar $p_w \in \mathbb{R}$ as  follows
\begin{equation}
%	\begin{align}
\label{eqn:uw}
		\uw{w}(t) = \uw{\sigma_{1}}(t-k+1)\uw{\sigma_{2}}(t-k+2)\cdots\uw{\sigma_{k}}(t)  %\forall t \in \mathbb{Z} \nonumber \\
	%	p_w&=p_{\sigma_1}p_{\sigma_2} \cdots p_{\sigma_k}.
%	\end{align}
\end{equation}
For an empty word $w= \epsilon$, we set $\uw{\epsilon}(t)=1$. % $p_{\epsilon}=1$.
%It is in our interests for the covariances of $\p_i(t),\p_j(t)$ to be independent of past values of $\p$ and for $\uw{w}(t)$, $\uw{v}$ to be essentially orthogonal for $w \ne v$, unless $w$ and $v$ are suffixes of one another. 
%
%Therefore, we will be using \emph{admissible scheduling sequences}. Note that, for a detailed explanation, the definition of  is 

If $\p$ is admissible, then $\uw{w},\uw{v}$ are jointly wide-sense stationary. Moreover, $\uw{w}(t)$ and $\uw{v}(t)$ are uncorrelated, if the last letters of $w$ and
$v$ are different, and 
$$E[\uw{w\sigma}^2(t)]=p_{\sigma} E[\uw{w}^2(t)]$$ 
for any $w \in \Sigma^{+}$, $\sigma \in \Sigma$. 
That is, $\p$ uniquely determines a collection of numbers $\{p_{\sigma}\}_{\sigma \in \Sigma}$. This latter collection will play an important role in the sequel. 
In particular, for $\p$ from \textbf{case(1)}, 
$p_i$ is the variance of $\p_i$, and for $\p$ from Example \textbf{case(2)},
$p_i$ is the probability  $P(\theta(t)=i)$, for all $i \in \Sigma$. 
%in this case $\uw{w}(t)$ and $\uw{v}(t)$ are uncorrelated for 
%$v \ne w$, $|v|=|w|$ conditionally on the $\sigma$-algebra 
%$\mathscr{F}^{\p,-}_{t}$ generated by the past values of $\{\p(s)\}_{s <t}$. 
%More precisely,  for any $w,v \in \Sigma^{*}$, $\sigma,\sigma^{'} \in \Sigma$, $\sigma \ne \sigma^{'}$,
%$t \in \mathbb{Z}$, 
%$$E[\uw{w\sigma}(t)\uw{v\sigma^{'}}(t) \mid \mathscr{F}^{\p,-}_{t} ]=0$$
%and there exist numbers 
%\begin{equation}
%\label{def:admis:pq}
%\{p_{\sigma}\}_{\sigma \in \Sigma}
%\end{equation}
% such that if $w\ne \epsilon$, then 
%  \begin{equation*}
%  %\label{gen:filt:ass_new:cond1:def1:eq1}
%  \begin{split}
%      & E[\uw{w\sigma}(t)\uw{v\sigma}(t) \mid \mathscr{F}^{\p,-}_{t} ] = 
%                                                                          p_{\sigma} \uw{w}(t-1)\uw{v}(t-1) %                                                                         \\
%    % &   E[\uw{w\sigma}(t)\uw{v\sigma^{'}}(t) \mid \mathscr{F}^{\p,-}_{t} ]=0, ~   %E[\uw{\sigma}(t)\uw{\sigma^{'}}(t) \mid \mathscr{F}^{\p,-}_{t} ]                                     =0
%      %\left\{\begin{array}{rl}
%      %                                                                    p_{\sigma} %\uw{w}(t-1)\uw{v}(t-1) & \sigma=\sigma^{'}  \mbox { and  $w \ne \epsilon$} \\
%     %                                                                     0 & \mbox{$$\sigma \ne %\sigma^{'}$} 
%     %                                                                     \end{array}\right. \\
%     %&  E[\uw{w\sigma}(t)\uw{\sigma^{'}}(t) \mid \mathscr{F}^{\p,-}_{t}] = \\
%     %&   \left\{\begin{array}{rl}
%     %                                                                     p_{\sigma} \uw{w}(t-1)  &% \sigma=\sigma^{'} \mbox{ and }  \\
%                                                                         % 0 & \mbox{otherwise}
                                                                         % \end{array}\right. \\
%     %& E[\uw{\sigma}(t)\uw{\sigma^{'}}(t) \mid \mathscr{F}^{\p,-}_{t}] = \begin{array}{rl}
     %                                                                     0 & \mbox{if } \sigma \ne \sigma^{'} 
     %                                                                     \end{array}
%  \end{split}
%  \end{equation*}
%for any infinite sequence $\underline{v}=\{\sigma_i \in \Sigma\}_{i=1}^{\infty}$, the process ${\uw{}}^{\underline{v}}: k \mapsto \uw{\sigma_1\cdots \sigma_k}(t)$ is wide-sense stationary, and for different infinite sequences t
%$\underline{v}_1 \ne \underline{v}_2$ the random variables ${\uw{}}^{\underline{v}_1}(k)$ and ${\uw{}}^{\underline{v}_2}(k)$ are uncorrelated for any $k$, such that the first $k$ elements of the two sequences are not all the same.
%The second condition is a technical one, which is not strictly speaking necessary. The last condition is 

Now let $\r$ be a stochastic ZMWSII process w.r.t. $\p$, and
% \subsection{Processes which are wide-stationary with respect to the scheduling}
%\label{Subsec:assumptions2}
%Next, we will discuss an extension of the notion of wide-sense stationarity. To this end, assume that
%$\p$ is admissible.
let $\{p_{\sigma}\}_{\sigma \in \Sigma}$  be the constants determined by $\p$ as explained above. In order to explain the significance of 
these assumptions, we
define the products
\begin{equation}
	\begin{aligned}\label{eqn:uw1}
%		\uw{w}(t) &= \textcolor{red}{\uw{\sigma_{1}}(t-k+1)\uw{\sigma_{2}}(t-k+2)\cdots\uw{\sigma_{k}}(t) } \\ %\forall t \in \mathbb{Z} \nonumber \\
		p_w&=p_{\sigma_1}p_{\sigma_2} \cdots p_{\sigma_k}
	\end{aligned}
\end{equation}
for any $w \in \Sigma^{+}$, $\sigma_i \in \Sigma$. For an empty word $w= \epsilon$, we set $p_{\epsilon}=1$.
For a stochastic process $\mathbf{r} \in \mathbb{R}^{\udim}$ and for each $\wordSet{*}$ we define the stochastic process $\zwr$ as
\begin{equation}\label{eqn:zwu}
	\zwr(t) = \mathbf{r}(t-|w|) \uw{w}(t-1)\frac{1}{\sqrt{p_{w}}},
\end{equation}
where $\uw{w}$ and $p_w$ are as in \eqref{eqn:uw} and \eqref{eqn:uw1}. For $w=\epsilon$, $\zwr(t)=\r(t)$.
The process $\zwr$ in \eqref{eqn:zwu} is interpreted as the product of the \emph{past} of $\r$ and $\p$.
The process $\zwr$ will be used as predictors for future values of $\r$ for various choices of $\r$. 

%\emph{Zero Mean Wide Sense Stationary with respect to inputs} process and \emph{Square integrable} process respectively, are used throughout the paper. The two definitions can be found in Appendix \ref{App:def}.
Now we will explain the motivation for the concept of
ZMWSII. Assume that  $\r$ is ZMWSII w.r.t. $\p$, then $\zwr(t)$ is wide-stationary and 
square-integrable for all $w \in \Sigma^{+}$. Moreover,
the covariances $\expect{\zwr(t)(\zvr(t))^{T}}$ do not depend on $t$. Furthermore,
$\zwr(t)$, $\zvr(t)$ are orthogonal, if $w$ is not a suffix of $v$ or vice versa.
Recall that we say that $w$ is a suffix of $v$, if $v=sw$ for some $s \in \Sigma^{*}$.
Moreover, when $w$ is suffix of $v$, then 
%In particular, from \cite[Lemma ]{PetreczkyBilinear} it follows that
%if $\mathbf{r}$ is ZMWSII w.r.t. $\p$, then
\begin{equation*}
\begin{aligned}
		& \expect{\zwr(t)(\zvr(t))^{T}} = \left\{ \begin{array}{ll} %\expect{\zsr(t)(\r(t))^{T}} & \text{if } w = sv \\
		\expect{\r(t)(\zsr(t))^{T}} & \text{if } v = sw \\
	\expect{\zsigr(t)(\zsigr(t))^{T}} & \text{if } v=w = \sigma s \\
		 %& \text{if neither} 
		\end{array} \right. \\
%		& \expect{\zwsigr(t)(\zvsigpr(t))^{T}} = \left\{ \begin{array}{ll}		%
%		\expect{\zwr(t)(\zvr(t))^{T}} & \hspace{-0.7em} \text{if } \sigma = \sigma \\
%		0 & \hspace{-0.7em} \text{if } \sigma \neq \sigma' \\
		%\end{array} \right. \\
%		& \text{If $|w| = |v|$ then the following definition can be applied} \\
%		& \expect{\zwr(t)(\zvr(t))^{T}} = \left\{ \begin{array}{ll} 
%		\expect{\zsigr(t)(\zsigr(t))^{T}} & \text{if } v=w = \sigma s \\
%		0 & \text{if } w \neq v \\
		%\end{array} \right.
\end{aligned}
\end{equation*}
That is, $\expect{\zwr(t)(\zvr(t))^{T}}$ depends only on the difference
of $w$ and $v$, i.e., on the prefix of $v$.  
This can be viewed as a generalization of wide-sense stationarity,
if the index $w$ and $v$ are viewed as additional multidimensional time instances, and
$\Sigma^{*}$ is viewed as an additional time-axis. 


%All the processes considered in this paper will be assumed to be ZMWSSI and SII process w.r.t. the scheduling process $\p$.  

%Using the concept of ZMWSSI process w.r.t. scheduling $\p$, we can formulate the main assumption regarding the process $(\mathbf{y},\p)$.
%\begin{Assumption}%[Assumption on the input and output process]
%	\label{asm:main}%
%	$\p$ is consider an admissible scheduling sequence (satisfies Definition \ref{asm:A1}), and 
%	$\mathbf{y}$ is a ZMWSSI and SII process w.r.t. $\p$ (satisfies Definition \ref{def:ZMWSSI} and Definition \ref{Defn:SII}).  
%\end{Assumption}


%Next, in the following section, we recall from \cite[Definition 2]{MejariCDC2019} the notion of a \emph{stationary} stochastic LPV-SSA representation of a process $\r$ without inputs.
